Explicit synchronous partitioned scheme for coupled reduced order models based on composite reduced bases

This paper formulates, analyzes, and demonstrates numerically a method for the partitioned solution of coupled interface problems involving combinations of projection-based reduced order models (ROM) and/or full order methods (FOMs). The method builds on the partitioned scheme developed in [1], which starts from a well-posed formulation of the coupled interface problem and uses its dual Schur complement to obtain an approximation of the interface flux. Explicit time integration of this problem decouples its subdomain equations and enables their independent solution on each subdomain. Extension of this partitioned scheme to coupled ROM-ROM or ROM-FOM problems required formulations with non-singular Schur complements. To obtain these problems, we project a well-posed coupled FOM-FOM problem onto a composite reduced basis comprising separate sets of basis vectors for the interface and interior variables, and use the interface reduced basis as a Lagrange multiplier. Our analysis confirms that the resulting coupled ROM-ROM and ROM-FOM problems have provably non-singular Schur complements, independent of the mesh size and the reduced basis size. In the ROM-FOM case, analysis shows that one can also use the interface FOM space as a Lagrange multiplier. We illustrate the theoretical and computational properties of the partitioned scheme through reproductive and predictive tests for a model advection-diffusion transmission problem.

==> sec_IVR_FullSubBasis.tex <==
\section{Extension of IVR to ROM-ROM/FEM couplings using full subdomain bases} 
%%%%
In this section we briefly review the extension of IVR to ROM-ROM and ROM-FOM couplings, developed in \cite{AdC:arxiv2021}. For brevity we only present the ROM-ROM case, as the ROM-FOM coupling is very similar.  

To obtain the coupled ROM-ROM problem, we apply the POD/Galerkin method to the coupled FOM-FOM problem \eqref{AdC:eq:Idx1System}. 
\subsection{POD background}


\subsection{IVR extension to ROM-ROM coupling}
During the offline stage
of the model reduction procedure,
we solve a monolithic FEM problem to collect a series of solution snapshots over the entire domain $\Omega$ and arrange them into a snapshot matrix $\overline{X}$. We then partition $\overline{X}$ into subdomain snapshot matrices $\overline{X}_j$ containing the finite element DoFs on $\Omega_j$, $j=1,2$. After zeroing all entries of $\overline{X}_j$ corresponding to the Dirichlet nodes in the finite element mesh we obtain the adjusted snapshot matrices $X_j$ and compute their SVD, i.e., $X_j = U_j\Sigma_j V^T_j$. The reduced basis on each subdomain is defined as the first $d$ left singular vectors of the adjusted snapshot matrix, where $d>0$ is an integer that depends on the desired ROM accuracy. We arrange these vectors in reduced basis matrices $\widetilde{\Phi}_j$, $j=1,2$. Because the columns of these matrices contain both the interior and interface DoFs on $\Omega_j$, in the literature they are usually referred to as the \emph{full subdomain bases}. 
%
To effect the projection of the coupled FOM-FOM problem \eqref{AdC:eq:Idx1System} onto the reduced basis we set 
%
\begin{equation}\label{AdC:eq:ansatz}
\bm{u}_i := \widetilde{\Phi}_i \bm{\tilde{u}}_i + \bm{\beta}_i;\quad i=1,2.
\end{equation}
%
The rows of $\bm{\beta}_i$ corresponding to non-Dirichlet nodes are set to $0$, while the rows corresponding to Dirichlet nodes on $\Gamma_i$ contain the values of the Dirichlet boundary data $g_i$ at these nodes; see \cite{AdC:GunzburgerBCs}. Note that the FEM coefficient vectors $\bm{u}_i$, the reduced order coefficient vectors $\bm{\tilde{u}}_i$, and the boundary vectors $\bm{\beta}_i$ are functions of the time.

Inserting \eqref{AdC:eq:ansatz} into \eqref{AdC:eq:Idx1System} and then multiplying the resulting subdomain equations on the left by $\widetilde{\Phi}_j^T$ yields the full subdomain basis monolithic ROM-ROM system:
%
\begin{align}\label{AdC:eq:GroupedRR}
\begin{bmatrix}
\widetilde{M}_1  & 0 &  \widetilde{G}_1^T \\
0 & \widetilde{M}_2 & -\widetilde{G}_2^T \\
\widetilde{G}_1 & -\widetilde{G}_2 & 0
\end{bmatrix}
\begin{bmatrix}
\bm{\dot{\tilde{u}}}_1 \\ \bm{\dot{\tilde{u}}}_2 \\ \bm{\lambda}
\end{bmatrix}
= \begin{bmatrix}
 \widetilde{\bm{f}}_1 - \widetilde{K}_1 \bm{\tilde{u}}_1 - \widetilde{\Phi}_1^T K_1 \bm{\beta}_1 -  \widetilde{\Phi}_1^T M_1 \bm{\dot{\beta}}_1  \\
 \widetilde{\bm{f}}_2 - \widetilde{K}_2 \bm{\tilde{u}}_2 - \widetilde{\Phi}_2^T K_2 \bm{\beta}_2 -  \widetilde{\Phi}_2^T M_2 \bm{\dot{\beta}}_2 \\
-G_1 \bm{\dot{\beta}}_1 + G_2 \bm{\dot{\beta}}_2 
\end{bmatrix}
=: \begin{bmatrix}
 \bm{s}_1 \\ \bm{s}_2 \\ 0
\end{bmatrix}
\end{align}
where $\widetilde{M}_i = \widetilde{\Phi}_i^T M_i \widetilde{\Phi}_i$, $\widetilde{K}_i = \widetilde{\Phi}_i^T K_i \widetilde{\Phi}_i$, $\widetilde{G}_i = G_i \widetilde{\Phi}_i$, and $\widetilde{\bm{f}}_i = \widetilde{\Phi}_i^T \bm{f}_i$. We note that the right-hand side of the last equation, $-G_1 \bm{\dot{\beta}}_1 + G_2 \bm{\dot{\beta}}_2$, is precisely zero, because the matrices $G_i$ act only on the interface nodes where the coefficients of $\bm{\beta}_i$ are zero by construction.  
 

Similar to the monolithic FOM-FOM problem \eqref{AdC:eq:Idx1System}, which is the basis for the IVR scheme, the monolithic  problem \eqref{AdC:eq:GroupedRR} is the basis for the extension of IVR to ROM-ROM couplings, which reads as follows.

\medskip
\noindent
\textbf{Offline: Computation of POD bases and and pre-computation of matrices for the full subdomain basis ROMs}
\medskip

\begin{enumerate}
\item Using a suitable monolithic FOM solve the model problem \eqref{AdC:strongForm} on $\Omega$, collect solution snapshots into a snapshot matrix $\overline{X}$ and partition $\overline{X}$ into subdomain snapshot matrices $\overline{X}_j$, $j=1,2$. Compute the SVD of the adjusted snapshot matrix $X_{j} = U_{j} \Sigma_{j} V^T_{j}$.
%
\item For $j=1,2$,  given a threshold $\delta_j >0$, define the reduced basis dimension $N_{R,j}$ as the smallest integers such that $\sum_{k=1}^{N_{R,j}} \sigma_{j,k}^2 \geq \Big(1 - \delta_j \Big)\sum_{k=1}^N \sigma_{j,k}^2 $, where $\sigma_{j,k}$ are the singular values from the diagonal of $\Sigma_j$, and $N$ is the total number of singular values.  Define the reduced basis matrices $\widetilde{\Phi}_{j}$ by retaining the first $N_{R,j}$ columns of $U_j$.
%
\item For $j=1,2$, precompute the ROM matrices, where $N_\gamma$ is the size of the LM space:
	\begin{align}\label{eq:projMatrices}
	\begin{split}
\widetilde{M_j}:=\widetilde{\Phi}_{j}^T M_j\widetilde{\Phi}_{j} \in &\mathbb{R}^{N_{R,j}\times N_{R,j}};\quad 
\widetilde{K}_j:= \widetilde{\Phi}_{j}^T K_j \widetilde{\Phi}_{j} \in \mathbb{R}^{N_{R,j}\times N_{R,j}};\\
&\quad\mbox{and}\quad \widetilde{G}_j:= G_j \widetilde{\Phi}_{j} \in \mathbb{R}^{N_{\gamma} \times N_{R,j}}\,.
\end{split}
	\end{align}
\end{enumerate} 

\medskip
\noindent
\textbf{Online: Solution of the full subdomain basis ROM-ROM system}
\begin{enumerate}
\medskip

\item Given a simulation time interval $[0,T]$ choose an explicit time integration scheme, or an IMEX scheme with explicit treatment of $\bm{\lambda}$, for each subdomain, i.e., an operator $D^n_{j,t}(\bm{\tilde{u}})$, $j=1,2$.
%
\item For $n=0,1,\ldots$ use $\bm{\tilde{u}}_1^n$ to compute the vector 
$$
\bm{s}_1^n :=\widetilde{\Phi}_{1}^T \mathbf{f}_1^n - \widetilde{K}_1\bm{\tilde{u}}_1^n - \widetilde{\Phi}^T_{1}K_1\bm{\beta}_1^n - \widetilde{\Phi}_1^T M_1 \bm{\dot{\beta}}_1^n
$$
\item For $n=0,1,\ldots$ use $\bm{\tilde{u}}_2^n$ to compute the vector 
$$
\bm{s}_2^n :=\widetilde{\Phi}_{2}^T \mathbf{f}_2^n - \widetilde{K}_2\bm{\tilde{u}}_2^n - \widetilde{\Phi}^T_{2}K_2\bm{\beta}_2^n - \widetilde{\Phi}^T_2 M_2 \bm{\dot{\beta}}_2^n.
$$
\item Solve the Schur complement system 
$$
\big( \widetilde{G}_1 \widetilde{M}_1^{-1} \widetilde{G}_1^T  + 
\widetilde{G}_2 \widetilde{M}_2^{-1} \widetilde{G}_2^T \big) \bm{\lambda}^n = 
\widetilde{G}_1 \widetilde{M}_1^{-1} \bm{s}_1^n -  
\widetilde{G}_2 \widetilde{M}_2^{-1}  \bm{s}_2^n
$$
for $\bm{\lambda}^n$. Compute $\widetilde{G}_1^T \bm{\lambda}^n$ and $\widetilde{G}_2^T \bm{\lambda}^n$.
 \item Solve the system $\widetilde{M}_1 D^n_{1,t}(\bm{\tilde{u}}_1) = \bm{s}_1^n - \widetilde{G}_1^T \bm{\lambda}^n$.
 \vspace{.25mm}
 \item Solve the system $\widetilde{M}_2 D^n_{2,t}(\bm{\tilde{u}}_2) = \bm{s}_2^n + \widetilde{G}_2^T \bm{\lambda}^n$.
 %
 \item Project the ROM solutions $\bm{\tilde{u}}_i$ onto the full order state spaces on $\Omega_i$, $i=1,2$:
 $$
 \bm{u}_1 := \widetilde{\Phi}_{1} \bm{\tilde{u}}_1 + \bm{\beta}_1; \quad
 \bm{u}_2 := \widetilde{\Phi}_{2} \bm{\tilde{u}}_2 + \bm{\beta}_2.
 $$
%
\end{enumerate}
%

%\begin{remark}
%The matrices appearing in the ROM systems, namely \eqref{eq:projMatrices}, can only be precomputed in the
%case of a linear partial differential equation (PDE).  For nonlinear problems, to circumvent the
%computational cost of computing the projection of the nonlinear terms in the PDEs onto the reduced basis online, 
%	hyper-reduction approaches such as the Discrete Empirical Interpolation Method (DEIM) \cite{AdC:DEIM}, gappy POD \cite{AdC:Gappy} and 
%	the Energy-Conserving Sampling and Weighting (ECSW) method \cite{AdC:ECSW} can be employed.  We will consider extensions of 
%our methods to nonlinear problems in a subsequent publication. \\
%\end{remark}

It is clear that success of the above extension of IVR to a ROM-ROM coupling hinges on the unique solvability of the Schur complement system in Step 4 of the \emph{online} portion of the scheme. For the original IVR scheme, one can show that under some conditions on the Lagrange multiplier space the dual Schur complement of the upper left 2 $\times$ 2 submatrix from \eqref{AdC:eq:Idx1System} is symmetric and positive definite; see \cite{AdC:CAMWA} for details. In particular, choosing the trace of the finite element space from either one of the subdomains as a Lagrange multiplier space always satisfies these conditions. 

At the same time, one can easily construct an example for which the matrix $\widetilde{S} := \widetilde{G}_1 \widetilde{M}_1^{-1} \widetilde{G}_1^T + \widetilde{G}_2 \widetilde{M}_2^{-1} \widetilde{G}_2^T$ cannot even be defined. To that end, it suffices to consider any manufactured solution whose restriction to $\Omega_i$ is supported on a compact subset $\omega_i\subset\Omega_i$ such that $\omega_i$ does not intersect any elements having nodes on the interface $\gamma$.  In this case, all the rows of the snapshot matrix corresponding to interfacial degrees of freedom would be exactly 0, which would result in $\widetilde{\Phi}_i$ being 0 on those same rows. It is easy to see that in this case the projected mass matrices $\widetilde{M}_{i}$ will be singular, and so the Schur complement will be undefined. 

The example problem used to perform reproductive tests of the full subdomain basis extensions of IVR to ROM-ROM and ROM-FOM in  \cite{AdC:arxiv2021} did not have the pathology described in the above scenario and we did not observe failures of these formulations. At the same time, these extensions of IVR obviously cannot offer any guarantees that the ROM-ROM and ROM-FOM couplings will be well-posed for all possible configurations of the model transmission problem \eqref{AdC:strongForm}. In the next section we formulate a modified version of the IVR extension that resolves this issue.


